Methods for Mitigating Uncertainty in Real-Time Operations of a Connected Microgrid

In this paper, we compare the effectiveness of a two-stage control strategy for the energy management system (EMS) of a grid-connected microgrid under uncertain solar irradiance and load demand using a real-world dataset from an island in Southeast Asia (SEA). The first stage computes a day-ahead commitment for power profile exchanged with the main grid, while the second stage focuses on real-time controls to minimize the system operating cost. Given the challenges in accurately forecasting solar irradiance for a long time horizon, scenario-based stochastic programming (SP) is considered for the first stage. For the second stage, as the most recent weather conditions can be used, several methodologies to handle the uncertainties are investigated, including: (1) the rule-based method historically deployed on EMS, (2) model predictive controller (MPC) using either an explicit forecast or scenario-based stochastic forecast, and (3) Deep Reinforcement Learning (DRL) computing its own implicit forecast through a distribution of costs. Performances of these methodologies are compared in terms of precision with a reference control assuming perfect forecast -- i.e. representing the minimal achievable operation cost in theory. Obtained results show that MPC with a stochastic forecast outperforms MPC with a simple deterministic prediction. This suggests that using an explicit forecast, even within a short time window, is challenging. Using weather conditions can, however, be more efficient, as demonstrated by DRL (with implicit forecast), outperforming MPC with stochastic forecast by 1.3\%.

==> sections/biography.tex <==
\newpage

\bio{}
Author biography without author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

\bio{figs/pic1}
Author biography with author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

\bio{figs/pic1}
Author biography with author photo.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
Author biography. Author biography. Author biography.
\endbio

==> sections/extras.tex <==
%%%%%%%%%%%%% CONSTRAINTS
% Power Balance
At any point in time, the generated energy must be greater than the demanded load, as shown in Eq. \ref{eq:power_balance}, provided the surplus energy can be curtailed and/or exported to the main grid. Note that in practice there shall be a balance between load and generation. Also, mathematically any surplus of generation would incur additional costs and therefore degrade the objective \aea{Why? What if I can export that energy to the main grid and earn?}. At the optimal point, the constraint in Eq. \ref{eq:power_balance} is always active (i.e. equality). Here $P^t_{sol}$ and $P^t_{dem}$ denote the solar power and load demand at time $t$, respectively.
\begin{equation}
    P^t_{dESS} - P^t_{cESS} + P^t_{sol} + P^t_{dg} + P^t_{gb} - P^t_{gs} \geq P^t_{dem} \quad \forall t \in T
    \label{eq:power_balance}
\end{equation}

% Grid Constraint
The import/export of electricity from/to the grid is bounded to $\overline{P}_g$, which is shown in equation \ref{eq:grid_constraint}. In any instance, the microgrid can only buy or sell energy from the main grid. $u^t_{g}$ is a binary variable that is $1$ for purchasing electricity from the grid and $0$ for selling electricity to the grid and constraints in equation 3 ensure that import and export do not occur simultaneously. \aea{Is $\overline{P}_g$ a parameter or variable? Not explained. In general, you need to define your case study setting up front, before diving into the problem. What are the components, what parameters are given, what are the control knobs, etc.}
\begin{equation}
    \begin{aligned} 
    0 &\leq P^t_{gb} \leq u^t_g \times \overline{P}_g & \quad \forall t \in T  \\
    0 &\leq P^t_{gs} \leq (1 - u^t_g) \times \overline{P}_g & \quad \forall t \in T
    \label{eq:grid_constraint}
\end{aligned}
\end{equation}

% Battery Constraint
The charging or discharging of ESS is constrained by $\overline{P}_{ ESS }$, where $u^t_{ ESS }$ denotes the charging mode, and Eq.\aea{Consistency please. Either Eq. or equation, not both.} \ref{eq:ess_constraint_bound} ensures that charging and discharging are complementary. Equation \ref{eq:ess_constraint_soc} updates the state of charge represented by the energy within the battery $E^t$, where $\eta_d$ and $\eta_c$ represent the efficiency of ESS discharge and charge, respectively. Equation \ref{eq:ess_constraint_end} ensures that the SOC at the end of the sliding window horizon is equal to $E_{end}$ \aea{What is SOC? What is $E_{end}$?}.
\begin{equation}
    \begin{aligned} \label{eq:ess_constraint_bound}
       0 &\leq P_{dESS} \leq u^t_{ESS} \times \overline{P}_{ESS} & \quad \forall t \in T \\
       0 &\leq P_{cESS} \leq (1 - u^t_{ESS}) \times \overline{P}_{ESS} & \quad \forall t \in T
    \end{aligned}
\end{equation}
\begin{equation} \label{eq:ess_constraint_soc}
   E^t = E^{t-1} - \eta_d P^t_{dESS} + \eta_c P^t_{cESS} \quad \forall t \in T
\end{equation}
\begin{equation} \label{eq:ess_constraint_end}
   E^T \geq E_{end}
\end{equation}

% Reserve Constraint    
To provide ancillary services \aea{Never explained.} (i.e. downward/upward regulation), we reserve a certain amount of ESS charge/discharge power, limited to the maximum power capacity of ESS $\overline{P}_{ ESS }$ given in Eq. \ref{eq:reserve_constraint_bound}. Equation \ref{eq:reserve_constraint_pow} ensures that the sum of the scheduled charge/discharge power ($P^t_{dESS}, P^t_{cESS}$) and the reserve power ($R^t_d$, $R^t_c$) does not exceed the maximum rated power of the ESS denoted $\overline{P}_{ ESS }$. Equation \ref{eq:reserve_constraint_soc} ensures that the reserve power should be within the available power of ESS.
\begin{equation}
   \begin{aligned} \label{eq:reserve_constraint_bound}
    R^t_d &\leq (1 - u^t_g) \times \overline{P}_{ESS} & \quad \forall t \in T \\
    R^t_c &\leq u^t_g \times \overline{P}_{ESS} & \quad \forall t \in T
\end{aligned} 
\end{equation}
\begin{equation}
    \begin{aligned} \label{eq:reserve_constraint_pow}
    R^t_d + P^t_{dESS} - P^t_{cESS} &\leq \overline{P}_{ESS} & \quad \forall t \in T \\
    R^t_c - P^t_{dESS} + P^t_{cESS} &\leq \overline{P}_{ESS} & \quad \forall t \in T
\end{aligned}
\end{equation}
\begin{equation}
    \begin{aligned}\label{eq:reserve_constraint_soc}
    \eta_d R^t_d &\leq E^t - \underline{E} & \quad \forall t \in T \\
    \eta_c R^t_c &\leq \overline{E} - E^t & \quad \forall t \in T
\end{aligned}
\end{equation}

% Generator
DG can be used to serve load demand when energy supply from other sources is inadequate. $\alpha^t_{dg}$ and $\beta^t_{dg}$ are the start and stop commands for DG. $u^t_{dg}$ is a binary variable that
represents the on/off status of the DG. Equations \ref{eq:dg_constraint_comm} and \ref{eq:dg_constraint_status} show the relationship between the start/stop command for the generator and the generator status at time $t$ --- i.e. start-up and shutdown cannot occur simultaneously, and a logical relationship between the on/off status and the
start/stop variables. Equation \ref{eq:dg_constraint_bound} sets a bound on the generator power by the generator maximum capacity $\overline{P}_{dg}$. Equation \ref{eq:dg_constraint_ramp} ensures that the power variation of the generator power over two successive time steps remains within the up ramp $RU$ and the down ramp $RD$ limits. In addition, the power variation is limited to a start-up ramp $SU$ and a shutdown ramp $SD$ when starting and stopping the generator.
\begin{equation}\label{eq:dg_constraint_comm}
    \alpha^t_{dg} + \beta^t_{dg} \leq 1 \quad \forall t \in T
\end{equation}
\begin{equation} \label{eq:dg_constraint_status}
    \alpha^t_{dg} - \beta^t_{dg} \leq u^t_{dg} - u^{t-1}_{dg} \quad \forall t \in T
\end{equation}
\begin{equation}
    \begin{aligned} \label{eq:dg_constraint_bound}
    P^t_{dg} &\leq u^t_{dg} \times \overline{P}_{dg} & \quad \forall t \in T \\
    P^t_{dg} &\geq u^t_{dg} \times \underline{P}_{dg} & \quad \forall t \in T
    \end{aligned} 
\end{equation}
\begin{equation}
   \begin{aligned} \label{eq:dg_constraint_ramp}
    P^t_{dg} - P^{t-1}_{dg} \leq u^{t-1}_{dg} \times RU + \alpha^t_{dg} \times SU & \quad \forall t \in T \\
    P^{t-1}_{dg} - P^t_{dg} \leq u^{t}_{dg} \times RD + \beta^t_{dg} \times SD & \quad \forall t \in T
\end{aligned} 
\end{equation}


\subsection{MPC for Real-Time Operation} \label{model:mpc}

In real-time operation, we adopt an MPC approach with a rolling horizon to strictly adhere to the day-ahead commitment with the main grid and minimize the operating cost, i.e., determine the optimal power profiles. MPC adjusts the ESS charge/discharge along with the DG power to ensure the cost-efficient operation and mitigate uncertainties.
The solution obtained for ESS charge/discharge $P^1_{dESS}$, $P^1_{cESS}$, and DG power $P^1_{dg}$ at $t=1$ (current time step) is used as the set-point for real-time operation, and solutions of other time steps are discarded, as is typically done in MPC. The objective for real-time operation is shown in Eq. \ref{eq:obj_real_time}, with the same constraints as those in Eqs. \ref{eq:power_balance} to \ref{eq:dg_constraint_ramp}, along with safety constraints in Eqs. \ref{eq:safety1} and \ref{eq:safety2}. To forecast solar generation and load demand, we use a strategy discussed in subsection \ref{model:forecast}.

\begin{multline} \label{eq:obj_real_time}
  \min_{\substack{P^0_{dESS}, P^0_{cESS} \\ P^0_{dg}}} 
  \sum_{t=1}^{T}{ \Biggl[ C_{gb}^t P_{gb}^{*t} - C_{gs}^t P^{*t}_{gs} - C_{r}^t R_{d}^{*t} - C_{r}^t R_{c}^{*t}  } \\
 + C_{ESS}^t P_{dESS}^t + C_{ESS}^t P_{cESS}^t + C_{dg}^t P_{dg}^t  \Biggr] 
\end{multline}


For safe operations in the presence of uncertainty, we use the constraint shown in Eq. \ref{eq:safety1} and \ref{eq:safety2} for real-time operation. The generator should be positioned in such a way at the present time step that it can fulfil the requirement for a worst-case load demand at the next time step denoted as $P_{wc}^{t+1}$.
\begin{multline} \label{eq:safety1}   
\overline{P}_{ESS} - R^{t+1}_d + P^t_{dg} + \alpha^{t+1}_{dg} SU \\
+ u^t_{dg} RU + P^{t+1}_{gb} - P^{t+1}_{gs} \geq P^{t+1}_{wc} 
\end{multline}

\begin{multline} \label{eq:safety2}   
E^t - \underline{P}_{ESS} - R^{t+1}_d + P^t_{dg} + \alpha^{t+1}_{dg} SU \\
+ u^t_{dg} RU + P^{t+1}_{gb} - P^{t+1}_{gs} \geq P^{t+1}_{wc} 
\end{multline}



\subsection{Stochastic Programming for Real-Time Operation} \label{model:sp}
Similar to the day-ahead contract generation, we use scenario-based Stochastic Programming for the real-time operation which is shown to handle uncertainties in multiple works of literature \cite{AKBARIDIBAVAR2020106425, SHOKRIGAZAFROUDI2019201}. 

\begin{multline} \label{eq:obj_real_time_sp}
  \min_{\substack{P^{0,0}_{dg}}}
  \sum_{s \in S_r} \pi_r(s)
  \sum_{t=1}^{T}{ \Biggl[ C_{gb}^{t} P_{gb}^{*t} - C_{gs}^t P^{*t}_{gs} - C_{r}^t R_{d}^{*t} - C_{r}^t R_{c}^{*t} } \\
  + C_{ESS}^{t} P_{dESS}^{s,t} + C_{ESS}^{t} P_{cESS}^{s,t} + C_{dg}^t P_{dg}^{s,t}  \Biggr] 
\end{multline}

We use the same constraints as in Eq. \ref{eq:power_balance} to \ref{eq:dg_constraint_ramp}. All the variables and input parameters are defined along the set of defined scenarios $S_r$ in Eq. \ref{eq:power_balance} and from Eq. \ref{eq:ess_constraint_bound} to \ref{eq:dg_constraint_ramp} --- i.e. $P_{dem}^{s, t}, P_{sol}^{s, t}, P_{cESS}^{s,t}, P_{cESS}^{s,t}, \alpha_{dg}^{s,t}, \beta_{dg}^{s,t}, u_{dg}^{s,t}$ and $P_{dg}^{s,t}$ with $s \in S_r$. $\pi_r(s)$ denotes the probability of each scenario $s \in S_r$, we assume it to be uniform. Additionally, the following two steps are implemented for real-time decision making:

\begin{enumerate}
    \item A constraint to set the generator power $P_{dg}^{s,0}$ at $t=0$ equal for all scenarios $s \in S_r$ as in Eq.\ref{eq:dg0_sp}. 
    \begin{equation}\label{eq:dg0_sp}
        P_{dg}^{s,0} = P_{dg}^{0,0}, \quad \forall s \in S_r
    \end{equation}
    \item Replace the demand and solar power $P_{dem}^{s, 0}, P_{sol}^{s, 0}$ at $t=0$ with the current value of demand and solar power, while the values for the subsequent time steps correspond to solar and demand profile of respective scenarios $s \in S_r$. Here, we don't use any forecasting algorithm as in subsection \ref{model:mpc} to forecast load demand and solar generation. Instead, we generate $|S_r|$ of solar generation and load demand profiles from the dataset using clustering.
\end{enumerate}

The real-time SP returns optimal profiles along the prediction horizon. The control values at the first time step are actually implemented --- i.e. the optimal set-point for the DG power $P_{dg}^{0,0}$ and the set-point of ESS charge/discharge power which is computed analytically in accord with surplus/deficit power in the microgrid.
    

\subsection{Rule-Based Real-Time Operation}\label{model:rule}
We use a cycle charge rule-based algorithm for the real-time operation as in \cite{dreem} to determine the start or stop sequences of the generator based on ESS SOC levels -- i.e. setpoints of $DG_{start}$ and $DG_{stop}$ respectively. Figure \ref{fig:rule_based} shows the state transition diagram of rule-based operation. $DG_{start}$ denotes battery SOC $E^t$ at which the generator should start and $DG_{stop}$ denotes battery SOC at which the generator should stop. Whenever the generator starts, it delivers a power set by default at the optimal capacity which is 75\% of full generator capacity. However, the generator setpoint is curtailed or increased according to the actual real-time power requirement. 
% DG ON: ESS is charged from excess solar and excess DG
% DG ON: Increase setpoint towards optimal capacity, but energy is curtailed according to the need, may not always recharge the ESS during DG ON

\begin{figure}[!htb]
    \centering
    \includegraphics[scale=0.8]{imgs/rule_based.pdf}
    \captionsetup{justification=centering}
    \caption{Rule-based real-time operation.}
    \label{fig:rule_based}
\end{figure}



\subsection{Deep Reinforcement Learning for Real-Time Operation}\label{model:rl}

Due to unavoidable forecast errors, the deployment plan obtained by MPC is subject to uncertainties that can degrade
the expected performances (i.e. cost) of the system and endanger the fulfilment of the committed profiles. In order to mitigate the impact of those uncertainties, the control that is actually sent to the DESs is computed in real-time with the use of Reinforcement Learning. Especially, a model-free Markov Decision Process (MDP) is implemented while considering tuples of "States", "Actions" and "Reward" $(S, A, R)$  \cite{sutton2018reinforcement}.

The set state (observations) $S$ is represented as a six-dimensional vector $\big< h, P^h_{dem}, P^h_{sol}, E^{h-1}, E^{0^{-}}, P^{h-1}_{dg} \big>$, where $h$ is the hour of the day (integer value). $P^h_{dem}$ and $P^h_{sol}$ denotes measured load demand and solar generation respectively. $E^{h-1}$ is SOC of ESS at the end of the previous hour and $E^{0^{-}}$ is SOC of ESS at midnight i.e. at 00 Hrs. $P^{h-1}_{dg}$ is the generator power at previous hour. The action set $A$ is a set of finite actions denoting the generator power. The reward function $R$ is the immediate reward received when the agent takes action $a_s \in A$ from a state $s \in S$ which is shown in Eq. \ref{reward}. In the considered implementation, the objective is then to avoid any blackouts while reducing the cost of operation $C(s, a_s)$ with a weighting factor of $w_b$ and $w_o$ respectively. A blackout occurs whenever the load is not satisfied with chosen action. 
\begin{equation} \label{reward}
  R(s, a_s) = -w_o \times C(s,a_s) -w_b \times 
    \begin{cases}
        1 &\text{for blackout}\\
        0 &\text{otherwise}
    \end{cases}
\end{equation}

Since the real-time actions are computed with a model-free MDP, we use DQN (Deep-Q Learning) \cite{mnih2015human} to train the agent to perform appropriate actions to maximize the total reward. DQN has been shown to outperform other DRL approaches for the microgrid applications related to the use case considered in our work \cite{dreem}. The DRL agent generates an hourly setpoint of DG power for real-time operation given the current state of the system. Once the system is controlled along the simulation horizon, performances of the proposed approach can be assessed.



\subsection{Solar Power and Load Demand Forecasting for MPC}\label{model:forecast}
For real-time operation using MPC, as previously discussed, rely on the forecast of solar generation and load demand for future $T$ time steps. In contrast to SP, where we use fixed solar and demand profiles for future values instead of forecasting in real-time. In order to assess the performance of the proposed control strategy, forecasts for demand and solar generation are emulated using a classical approach called exponential moving averaging (EMA) \cite{ema}. As shown in Eq. \ref{eq:ema}, where, $y^{t}$ denotes the moving average at present time instance, $x^{t}$ denotes the present value and $\theta$ denotes the smoothing constant. Here, $y^{t+1}$ is considered as the forecasted value for the next step. 


\begin{equation}\label{eq:ema}
    y^{t+1} = \theta \times y^{t} + (1-\theta) \times x^{t}
\end{equation}

Eq. \ref{eq:ema} is used to forecast solar generation and load demand for a certain time of day by taking into account the historical data of solar generation/load demand at the same time of day. For instance, to forecast solar/demand power at 8 AM tomorrow, historical data of solar generation/load demand only at 8 AM till today is used to compute EMA.

\begin{equation}\label{eq:scale}
    sf^{t+1} = \frac{1}{\sum_{j=0}^{j=2} (\kappa)^{j+1}} \sum_{j=0}^{j=2} 
    \Biggl[
    (\kappa)^{j+1} \times
    \begin{cases}
        \frac{ x^{t-j}}{y^{t-j} },& \text{if }  y^{t-j} > 0 \\
         1,              & \text{otherwise}
    \end{cases}
    \Biggl]
\end{equation}

To improve the accuracy of solar generation and load demand forecasting with EMA, we introduce a scaling factor denoted as $sf^{t+1}$. It helps to capture information about how well the EMA's prediction is performing for recent predictions. In this work, we compute the scaling factor based on the last three predictions $y^{t-2}$, $y^{t-1}$, and $y^t$ to improve the accuracy of prediction. It's important to note that the choice of the number of past predictions to compute the scaling factor can vary depending on the specific forecasting problem and the nature of the data. Eq. \ref{eq:scale} is used to compute the scaling factor where $\kappa$ is a constant weighing factor to give more preference to more recent local data. The forecast is obtained by multiplying the EMA forecasted solar generation/load demand value with the scaling factor $sf^{t+1}$.

==> sections/related.tex <==
\section{Related Work} \label{related_work}
A vast amount of research in the area of microgrid operations focuses on uncertainty mitigation through appropriate scheduling and power allocation of DERs, i.e., deciding when and how much energy to use from specific DERs \cite{SOLEYMANI20081493, SHOKRIGAZAFROUDI2019201}.

EMSs then often rely on forecasts of renewable generation and load demand to optimize DER dispatch, although several research papers propose methods that do not require any forecast \cite{PRATHAPANENI2019100232}. However, a forecast-based approach is applied for real-time operation and optimization in microgrids for its compute efficiency and simplicity \cite{meng2016microgrid, FATHIMA2015431, SHARMA2022120028}. Traditional optimization approaches use forecast-based strategies to formulate the microgrid operation as a mathematical program such as linear program (LP), Mixed Integer Linear Program (MILP), Mixed Integer Non-Linear Program (MINLP), etc. \cite{meng2016microgrid, en11010129, liu2011hybrid, tse2015, tpe2017}. Some related studies also solve this problem using heuristic optimization methods such as genetic algorithm, simulated annealing algorithm, particle swarm optimization and ant colony optimization \cite{tste2010, SHARMA2022120028, FATHIMA2015431, MARZBAND2016265}, and even game theory when several stakeholders are involved \cite{tcdics2017}.


As already mentioned, one main difficulty in optimizing the operation of (micro) grids \cite{zhao2015, SHOKRIGAZAFROUDI2019201} is the uncertain demand and renewable power generation profiles. To mitigate those uncertainties, studies often employ strategies like Robust optimization or Stochastic Programming, chance-constraint methods, Monte Carlo simulations, etc. \cite{PRATHAPANENI2019100232, AKBARIDIBAVAR2020106425, SHOKRIGAZAFROUDI2019201}. Nevertheless, these strategies require the expected values or potential scenarios for  solar generation and load demand, which is often challenging to obtain accurately. Current research focuses on using data-driven, learning-based strategies such as reinforcement learning (RL) to alleviate the need for explicit forecasts. As promising examples, \cite{ji2019real} \cite{NAKABI2021100413} \cite{jpes2022} have applied Deep Reinforcement Learning (DRL) to optimize the economic dispatch in microgrids or \cite{isgte2019, dreem} proposed similar method for an islanded microgrid. Apart from the application of DRL in EMS, DRL has also been applied to other microgrid challenges, such as load management, demand response planning, and distributed energy management \cite{mocanu2018line, tsg2020, tsg2021, tps2018, zhou2020combined}.


Our study then compares various representative strategies for real-time operation in a two-stage optimization setup for a grid-connected microgrid, which is elaborately discussed in the following Section \ref{mgrid_dispatch}. We analyze the effectiveness of each strategy in handling uncertainties using a real-world dataset from SEA and provide conclusive remarks on their performance in Section \ref{result}.


